An enhancement of the fast time-domain boundary element method for the three-dimensional wave equation

Our objective is to stabilise and accelerate the time-domain boundary element method (TDBEM) for the three-dimensional wave equation. To overcome the potential time instability, we considered using the Burton--Miller-type boundary integral equation (BMBIE) instead of the ordinary boundary integral equation (OBIE), which consists of the single- and double-layer potentials. In addition, we introduced a smooth temporal basis, i.e. the B-spline temporal basis of order $d$, whereas $d=1$ was used together with the OBIE in a previous study [Takahashi 2014]. Corresponding to these new techniques, we generalised the interpolation-based fast multipole method that was developed in \cite{takahashi2014}. In particular, we constructed the multipole-to-local formula (M2L) so that even for $d\ge 2$ we can maintain the computational complexity of the entire algorithm, i.e. $O(N_{\rm s}^{1+\delta} N_{\rm t})$, where $N_{\rm s}$ and $N_{\rm t}$ denote the number of boundary elements and the number of time steps, respectively, and $\delta$ is theoretically estimated as $1/3$ or $1/2$. The numerical examples indicated that the BMBIE is indispensable for solving the homogeneous Dirichlet problem, but the order $d$ cannot exceed 1 owing to the doubtful cancellation of significant digits when calculating the corresponding layer potentials. In regard to the homogeneous Neumann problem, the previous TDBEM based on the OBIE with $d=1$ can be unstable, whereas it was found that the BMBIE with $d=2$ can be stable and accurate. The present study will enhance the usefulness of the TDBEM for 3D scalar wave problems.

==> Makefile <==
#SRC = main.tex
SRC = ms.tex

TEX = platex
#TEX = latex
#TEX = pdflatex
XDVI = pxdvi
DVIPS = pdvips
DVIPDFM = dvipdfmx

BIB = wave3d_paper.bib
AUX = ${SRC:.tex=.aux}
PDF = ${SRC:.tex=.pdf}

yymmdd = $(shell date +%y%m%d_%H%M)

#go: all
all: ${SRC} ${BIB} 
	${TEX} ${SRC}
#	makeindex ${SRC:.tex=.nlo} -s nomencl.ist -o ${SRC:.tex=.nls}
#	${TEX} ${SRC}
#	bibtex ${AUX}
#	${TEX} ${SRC}
	dvipdfmx ${SRC:.tex=.dvi}
clean:
	rm -f *.dvi *.log *.aux *.lot *.lof *.toc *.bbl *.blg *.spl *.out core
tar:
	#tar cvfz ${SRC:.tex=.tgz} Makefile *.tex *.bib *.sty *.bst
	tar cvfz ${SRC:.tex=.tgz} Makefile *.tex *.bib *.sty
euc:
	./sjis2euc.sh *.tex *.sty
sjis:
	./euc2sjis.sh *.tex *.sty
b back backup: tar
	mv ${SRC:.tex=.tgz} backup/${yymmdd}.tgz
	cp -p ${PDF} backup/${yymmdd}.pdf
copy:
	rsync -p 133.6.61.105:/home/ttaka/study/isoel2d/190219/shapeopt/test_circle/*.eps .

response:
	rm -f tmptmptmp*.pdf
	pdfseparate ${PDF} -f 34 -l 34 tmptmptmp%d.pdf
	pdfunite tmptmptmp*.pdf response.pdf
	rm -f tmptmptmp*.pdf
source:
	tar cvfz source.tar.gz \
	Makefile \
	app.tex biem.tex conclusion.tex element_integral.tex fmm2.tex introduction.tex linear.tex m2l_rec.tex m2l.tex ms.tex mydef.tex num.tex simplify.tex sphere_neumann2.tex \
	pmbb-sym.sty elsarticle-num-cpc.bst elsarticle.cls elsarticle \
	wave3d_paper.bib \
	bwefg-F-G.pgf  bwefg-J.pgf \
	figure/{*.eps,*.pgf,*.txt} \
	ms.bbl



==> elsarticle/doc/tmp.tex <==
 \begin{enumerate}[Step 1.]
  \item This is the first step of the example list.
  \item Obviously this is the second step.
  \item The final step to wind up this example.
 \end{enumerate}

